An Ecosystem for Personal Knowledge Graphs: A Survey and Research Roadmap

This paper presents an ecosystem for personal knowledge graphs (PKGs), commonly defined as resources of structured information about entities related to an individual, their attributes, and the relations between them. PKGs are a key enabler of secure and sophisticated personal data management and personalized services. However, there are challenges that need to be addressed before PKGs can achieve widespread adoption. One of the fundamental challenges is the very definition of what constitutes a PKG, as there are multiple interpretations of the term. We propose our own definition of a PKG, emphasizing the aspects of (1) data ownership by a single individual and (2) the delivery of personalized services as the primary purpose. We further argue that a holistic view of PKGs is needed to unlock their full potential, and propose a unified framework for PKGs, where the PKG is a part of a larger ecosystem with clear interfaces towards data services and data sources. A comprehensive survey and synthesis of existing work is conducted, with a mapping of the surveyed work into the proposed unified ecosystem. Finally, we identify open challenges and research opportunities for the ecosystem as a whole, as well as for the specific aspects of PKGs, which include population, representation and management, and utilization.

==> pkg-arch.tex <==

\begin{tikzpicture}[
  scale=1,
  xscale=1,
  yscale=.85
  ]

  \def\distX{4.5}
  \def\distY{2.7}

  \def\boxsize{1.3}

  \node[database, fill=blue!25] (pkg) at (0,-1) {PKG};

  
  \draw[round] (-\boxsize,-1-\boxsize) rectangle (\boxsize,-1+\boxsize);
  \node[white] at (0,-1-\boxsize) {\tabl{PKG mng system}};

  
  \node[database,fill=yellow!25] (lod) at (-\distX,  \distY) {};
  \node                                 at (-\distX,  \distY) {\tabl{Linked\\Open Data\\sources}};
  \node[database,fill=yellow!25] (ext2) at (-\distX,  0)      {};                           
  \node                                 at (-\distX,  0)      {\tabl{Public\\data\\sources}};
  \node[database] (ext1)                at (-\distX, -\distY) {};                             
  \node                                 at (-\distX, -\distY) {\tabl{Private\\data\\sources}};

  \draw[round] (-\distX-\boxsize,-\distY-\boxsize) rectangle (-\distX+\boxsize,\distY+\boxsize);
  \node[white] at (-\distX,\distY+\boxsize) {PKG data sources};
  
  \node[ontology] (kb1)                 at (0,\distY)         {Ontologies};
  
  \node[service] (ser1)                 at (\distX, 0)        {};
  \node                                 at (\distX, 0)        {Services};
  
  \node[user] (owner)                   at (\distX, -\distY)  {Owner};

  \node[circle,draw,minimum size=18mm,fill=blue!5] (outsidedata) at (1.7*\distX,  \distY) {Data};
  \node[user] (user)                                             at (1.7*\distX, -\distY) {Users};

  \draw[latex-] (lod) to [bend right=-0] node[iservice] {integrate} (kb1);
  \draw[-latex] (lod) to [bend right=-0] node[iservice] {integrate} (pkg);
  \draw[latex-] (pkg) to [bend right=0]  node[iservice] {integrate} (kb1);
  \draw[-latex] (-\distX+\boxsize,0) to [bend right=0] node[iservice] (extract1) {populate} (pkg);
  \draw[-latex] (pkg) to [bend right=-0] node[iservice] (sync) {synchronize} (ext1);

  \draw[latex-latex] (pkg) to [bend right=0] node[iservice] (read) {r/w access} (ser1);
  

  \draw[latex-] (ser1) to [bend right=0] node[iservice] () {import} (outsidedata);
  \draw[latex-latex] (ser1) to [bend right=0] node[iservice] () {utilize} (user);
  \draw[latex-latex] (ser1) to [bend right=0] node[iservice] () {utilize} (owner);
  \draw[latex-] (\boxsize,-1*\boxsize) to [bend right=0] node[iservice] (admin) {administrate} (owner);

  % bottom line
  \def\lp{-\distY-1.4*\boxsize}

  \draw (-\distX-1.2*\boxsize,\lp) to node[white] {population}                             (-1.7,\lp);
  \draw (-1.5,\lp) to node[white] {\tabl{representation\\and management}}  (1.5 ,\lp);
  \draw (1.7 ,\lp) to node[white] {utilization}                            (9   ,\lp);

  
\end{tikzpicture}


